Hidden assumptions of integer ratio analyses in bioacoustics and music

Rhythm is ubiquitous in human culture and in nature, but hard to capture in all its complexity. A key dimension of rhythm, integer ratio categories occur when the relationship between temporal intervals can be expressed as small-integer ratios. Recent work has found integer ratio categories in most human musical cultures and some animal species' vocalizations or behavioral displays. But biological systems are noisy, and empirically measured intervals rarely form an exact small-integer ratio. Here, we mathematically assess whether the leading integer ratio analysis method makes valid statistical and biological assumptions. In particular, we (1) make the temporal properties of empirical ratios explicit, both in general and for the typical use in the literature; (2) show how the choice of ratio formula affects the probability distribution of rhythm ratios and ensuing statistical results; (3) guide the reader to carefully consider the assumptions and null hypotheses of the statistical analysis; (4) present a comprehensive methodology to statistically test integer ratios for any null hypothesis of choice. Our observations have implications for both past and future research in music cognition and animal behavior: They suggest how to interpret past findings and provide tools to choose the correct null hypotheses in future empirical work.

==> main_aux.tex <==



==> supplement_aux.tex <==


